Flexible and Low-Complexity Encoding and Decoding of Systematic Polar Codes

In this work, we present hardware and software implementations of flexible polar systematic encoders and decoders. The proposed implementations operate on polar codes of any length less than a maximum and of any rate. We describe the low-complexity, highly parallel, and flexible systematic-encoding algorithm that we use and prove its correctness. Our hardware implementation results show that the overhead of adding code rate and length flexibility is little, and the impact on operation latency minor compared to code-specific versions. Finally, the flexible software encoder and decoder implementations are also shown to be able to maintain high throughput and low latency.

==> tikzlibrarymux.code.tex <==
% Define default style for this node
\tikzset{every mux2 node/.style={draw,minimum width=0.6cm,minimum height=2cm,inner sep=1mm,outer sep=0pt}}
\tikzset{every mux3 node/.style={draw,minimum width=0.6cm,minimum height=3cm,inner sep=1mm,outer sep=0pt}}
\tikzset{every mux4 node/.style={draw,minimum width=0.6cm,minimum height=4cm,inner sep=1mm,outer sep=0pt}}
\tikzset{every mux5 node/.style={draw,minimum width=0.6cm,minimum height=4.8cm,inner sep=1mm,outer sep=0pt}}

\pgfdeclareshape{mux2}{

  % The 'minimum width' and 'minimum height' keys, not the content, determine
  % the size
  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  % This is redundant, but makes some things easier:
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  % Inherit from rectangle
  \inheritanchorborder[from=rectangle]
  
  % Define same anchor a normal rectangle has
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{
    \pgf@process{\northeast}%
    \pgf@y=.25\pgf@y%
  }
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  \anchor{in0}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.5\pgf@y%
  }
  \anchor{in1}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.5\pgf@y%
  }
  \anchor{sel}{
    \pgf@process{\northeast}%
    \pgf@x=0pt%
    \pgf@y=-0.75\pgf@y%
  }

  \anchor{out}{
    \pgf@process{\northeast}%
    \pgf@y=0pt%
  }

  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
%
    \let\pgf@xnw=\pgf@xa
    \let\pgf@ynw=\pgf@yb
%
    \let\pgf@xsw=\pgf@xa
    \let\pgf@ysw=\pgf@ya
%
    \let\pgf@xse=\pgf@xb
    \pgf@yc=-\pgf@yb
    \advance\pgf@yc by \pgfshapeminwidth
    \let\pgf@yse=\pgf@yc
%
    \let\pgf@xne=\pgf@xb
    \pgf@xc=\pgf@yb
    \advance\pgf@xc by -\pgfshapeminwidth
    \let\pgf@yne=\pgf@xc
%
    \pgfpathmoveto{\pgfpoint{\pgf@xnw}{\pgf@ynw}}
    \pgfpathlineto{\pgfpoint{\pgf@xsw}{\pgf@ysw}}
    \pgfpathlineto{\pgfpoint{\pgf@xse}{\pgf@yse}}
    \pgfpathlineto{\pgfpoint{\pgf@xne}{\pgf@yne}}
    \pgfpathclose
    % Rectangle box
    %\pgfpathrectanglecorners{\southwest}{\northeast}
  }
}

\pgfdeclareshape{mux3}{

  % The 'minimum width' and 'minimum height' keys, not the content, determine
  % the size
  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  % This is redundant, but makes some things easier:
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  % Inherit from rectangle
  \inheritanchorborder[from=rectangle]
  
  % Define same anchor a normal rectangle has
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{
    \pgf@process{\northeast}%
    \pgf@y=.25\pgf@y%
  }
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  \anchor{in0}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.5\pgf@y%
  }
  \anchor{in1}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=0pt%
  }
  \anchor{in2}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.5\pgf@y%
  }
  \anchor{sel}{
    \pgf@process{\northeast}%
    \pgf@x=0pt%
    \pgf@y=-0.75\pgf@y%
  }

  \anchor{out}{
    \pgf@process{\northeast}%
    \pgf@y=0pt%
  }

  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
%
    \let\pgf@xnw=\pgf@xa
    \let\pgf@ynw=\pgf@yb
%
    \let\pgf@xsw=\pgf@xa
    \let\pgf@ysw=\pgf@ya
%
    \let\pgf@xse=\pgf@xb
    \pgf@yc=-\pgf@yb
    \advance\pgf@yc by \pgfshapeminwidth
    \let\pgf@yse=\pgf@yc
%
    \let\pgf@xne=\pgf@xb
    \pgf@xc=\pgf@yb
    \advance\pgf@xc by -\pgfshapeminwidth
    \let\pgf@yne=\pgf@xc
%
    \pgfpathmoveto{\pgfpoint{\pgf@xnw}{\pgf@ynw}}
    \pgfpathlineto{\pgfpoint{\pgf@xsw}{\pgf@ysw}}
    \pgfpathlineto{\pgfpoint{\pgf@xse}{\pgf@yse}}
    \pgfpathlineto{\pgfpoint{\pgf@xne}{\pgf@yne}}
    \pgfpathclose
    % Rectangle box
    %\pgfpathrectanglecorners{\southwest}{\northeast}
  }
}

\pgfdeclareshape{mux4}{

  % The 'minimum width' and 'minimum height' keys, not the content, determine
  % the size
  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  % This is redundant, but makes some things easier:
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  % Inherit from rectangle
  \inheritanchorborder[from=rectangle]
  
  % Define same anchor a normal rectangle has
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{
    \pgf@process{\northeast}%
    \pgf@y=.25\pgf@y%
  }
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  \anchor{in0}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.6\pgf@y%
  }
  \anchor{in1}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=0.2\pgf@y%
  }
  \anchor{in2}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.2\pgf@y%
  }
  \anchor{in3}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.6\pgf@y%
  }
  \anchor{sel}{
    \pgf@process{\northeast}%
    \pgf@x=0pt%
    \pgf@y=-0.75\pgf@y%
  }

  \anchor{out}{
    \pgf@process{\northeast}%
    \pgf@y=0pt%
  }

  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
%
    \let\pgf@xnw=\pgf@xa
    \let\pgf@ynw=\pgf@yb
%
    \let\pgf@xsw=\pgf@xa
    \let\pgf@ysw=\pgf@ya
%
    \let\pgf@xse=\pgf@xb
    \pgf@yc=-\pgf@yb
    \advance\pgf@yc by \pgfshapeminwidth
    \let\pgf@yse=\pgf@yc
%
    \let\pgf@xne=\pgf@xb
    \pgf@xc=\pgf@yb
    \advance\pgf@xc by -\pgfshapeminwidth
    \let\pgf@yne=\pgf@xc
%
    \pgfpathmoveto{\pgfpoint{\pgf@xnw}{\pgf@ynw}}
    \pgfpathlineto{\pgfpoint{\pgf@xsw}{\pgf@ysw}}
    \pgfpathlineto{\pgfpoint{\pgf@xse}{\pgf@yse}}
    \pgfpathlineto{\pgfpoint{\pgf@xne}{\pgf@yne}}
    \pgfpathclose
  }
}

\pgfdeclareshape{mux5}{

  % The 'minimum width' and 'minimum height' keys, not the content, determine
  % the size
  \savedanchor\northeast{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=0.5\pgf@x
    \pgf@y=0.5\pgf@y
  }
  % This is redundant, but makes some things easier:
  \savedanchor\southwest{%
    \pgfmathsetlength\pgf@x{\pgfshapeminwidth}%
    \pgfmathsetlength\pgf@y{\pgfshapeminheight}%
    \pgf@x=-0.5\pgf@x
    \pgf@y=-0.5\pgf@y
  }
  % Inherit from rectangle
  \inheritanchorborder[from=rectangle]
  
  % Define same anchor a normal rectangle has
  \anchor{center}{\pgfpointorigin}
  \anchor{north}{\northeast \pgf@x=0pt}
  \anchor{east}{\northeast \pgf@y=0pt}
  \anchor{south}{\southwest \pgf@x=0pt}
  \anchor{west}{\southwest \pgf@y=0pt}
  \anchor{north east}{
    \pgf@process{\northeast}%
    \pgf@y=.25\pgf@y%
  }
  \anchor{north west}{\northeast \pgf@x=-\pgf@x}
  \anchor{south west}{\southwest}
  \anchor{south east}{\southwest \pgf@x=-\pgf@x}
  \anchor{text}{
    \pgfpointorigin
    \advance\pgf@x by -.5\wd\pgfnodeparttextbox%
    \advance\pgf@y by -.5\ht\pgfnodeparttextbox%
    \advance\pgf@y by +.5\dp\pgfnodeparttextbox%
  }

  \anchor{in0}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=.7\pgf@y%
  }
  \anchor{in1}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=0.35\pgf@y%
  }
  \anchor{in2}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=0\pgf@y%
  }
  \anchor{in3}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.35\pgf@y%
  }
  \anchor{in4}{
    \pgf@process{\northeast}%
    \pgf@x=-1\pgf@x%
    \pgf@y=-.7\pgf@y%
  }
  \anchor{sel}{
    \pgf@process{\northeast}%
    \pgf@x=0pt%
    \pgf@y=-0.75\pgf@y%
  }

  \anchor{out}{
    \pgf@process{\northeast}%
    \pgf@y=0pt%
  }

  \backgroundpath{
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
%
    \let\pgf@xnw=\pgf@xa
    \let\pgf@ynw=\pgf@yb
%
    \let\pgf@xsw=\pgf@xa
    \let\pgf@ysw=\pgf@ya
%
    \let\pgf@xse=\pgf@xb
    \pgf@yc=-\pgf@yb
    \advance\pgf@yc by \pgfshapeminwidth
    \let\pgf@yse=\pgf@yc
%
    \let\pgf@xne=\pgf@xb
    \pgf@xc=\pgf@yb
    \advance\pgf@xc by -\pgfshapeminwidth
    \let\pgf@yne=\pgf@xc
%
    \pgfpathmoveto{\pgfpoint{\pgf@xnw}{\pgf@ynw}}
    \pgfpathlineto{\pgfpoint{\pgf@xsw}{\pgf@ysw}}
    \pgfpathlineto{\pgfpoint{\pgf@xse}{\pgf@yse}}
    \pgfpathlineto{\pgfpoint{\pgf@xne}{\pgf@yne}}
    \pgfpathclose
  }
}

